Differentially private Bayesian tests

Differential privacy has emerged as an significant cornerstone in the realm of scientific hypothesis testing utilizing confidential data. In reporting scientific discoveries, Bayesian tests are widely adopted since they effectively circumnavigate the key criticisms of P-values, namely, lack of interpretability and inability to quantify evidence in support of the competing hypotheses. We present a novel differentially private Bayesian hypotheses testing framework that arise naturally under a principled data generative mechanism, inherently maintaining the interpretability of the resulting inferences. Furthermore, by focusing on differentially private Bayes factors based on widely used test statistics, we circumvent the need to model the complete data generative mechanism and ensure substantial computational benefits. We also provide a set of sufficient conditions to establish results on Bayes factor consistency under the proposed framework. The utility of the devised technology is showcased via several numerical experiments.

==> backup.tex <==
\section{Differentially Private Bayes Factors Based on Test Statistics}
\textcolor{red}{Need to introduce the confluent hypergeometric functions, along with a reference, before we state the expresssions of the Bayes Factors.}

Consider a randomized mechanism $M: \mathcal{D} \rightarrow \mathbb{R}$ which satisfies $(\epsilon, \delta)$ differential privacy. For any data $d \in \mathcal{D}$, the mechanism can be mathematically expressed as
\begin{equation}\label{eqn:2.1}
    M(d) = f(d) + \eta,
\end{equation}
where $\eta$ is a privacy noise obtained via Gaussian or Laplace mechanism. It's important to emphasize that when determining the scale or rate parameters for the Gaussian or Laplace mechanism, careful selection is required to ensure the preservation of differential privacy. Consider the parameter of interest, denoted as $\theta$. In this context, we are regarding $f$ as a common test statistic , i.e $z$, $t$, $\chi^2$, $F$, etc.   It's worth noting that we can determine the density function of $M(d)$ through a convolution process, which can be expressed as follows:
$g(m \mid \theta) = \int_\eta u_\theta(m-\eta) p(\eta) d\eta$.
In this equation, $u(\cdot)$ represents the density function of the original test statistic, which is denoted as $f$, and $p(\cdot)$ is the density function of $\eta$. The marginal distribution of $M$ when the parameter $\theta$ is set to 0 in the null hypothesis is denoted as $g(m|\theta=0)$. However, in the alternative scenario, and assuming a non-local prior on $\theta$ as described in Johnson (2010), the marginal distribution of $M$ can be computed as follows: $m_1(m) = \int_\theta g(m \mid \theta) \pi(\theta) d\theta$. Here, $\pi(.)$ represents a non-local prior density function for the parameter $\theta$.

\begin{proposition}[$z$-test]\label{eqn:bfbot_z}
Assume that the distribution of the test statistic $f$ in \eqref{eqn:2.1}, under the null and the alternative hypothesis are described as
\begin{align*}
   \mbox{H}_0: f\ \sim\ \mbox{N}(0, 1),\quad \text{against}\quad 
   \mbox{H}_1: f\mid \theta \ \sim\ \mbox{N}(\theta, 1), \quad \theta\mid \tau^2 \sim J(\tau^2, r), \quad \tau>0, \quad r \geq 1,
\end{align*}
\begin{comment}
\begin{eqnarray}
H_0: f &\sim& N(0,1), \\
H_1: f| \theta &\sim& N(\theta,1), \qquad \theta| \tau^2 \sim J(\tau^2, r), \quad \tau>0, \quad r \geq 1,
 \end{eqnarray}
\end{comment}
respectively. Then, (i) the marginal distribution of $M$ under $\mbox{H}_1$ can be expressed as:
\begin{eqnarray}
     m_1(m) = \int \frac{\exp\big(-\frac{(m-\eta)^2}{2}\big)}{\sqrt{2\pi}(1+\tau^2)^{r+\frac{1}{2}}}\ {_1}F_1\Big(r + \frac{1}{2},\ \frac{1}{2},\ \frac{\tau^2 (m-\eta)^2}{2(1+\tau^2)}\Big)\ p(\eta) \ d\eta,\notag
 \end{eqnarray}
and (ii) the marginal distribution of M under the $\mbox{H}_0$ is given by:
\begin{eqnarray}
     m_0(m) = \int \frac{1}{\sqrt{2\pi}}\exp\big(-\frac{(m-\eta)^2}{2}\big)\ p(\eta) \ d\eta\notag.
\end{eqnarray}
\end{proposition}
\textcolor{red}{Does it yield a closed form expression under the Gaussian mechanism? If yes, we can include that as a remark. This comment holds for the next 3 lemmas as well.}

\begin{proposition}[$t$-test]\label{eqn:bfbot_t}
    Assume that the distribution of the test statistic $f$ in \eqref{eqn:2.1} under the null and the alternative hypothesis are described as
\begin{align*}
    \mbox{H}_0:  f\ \sim\ T_\nu ,\quad \text{against}\quad \mbox{H}_1: f\mid\theta\ \sim\ T_\nu (\theta), \quad \theta\mid \tau^2\ \sim\ J(\tau^2, r), \quad \tau>0, \quad r \geq 1,
\end{align*}
respectively. Then, (i)
\begin{comment}
\begin{eqnarray}
H_0: f &\sim& T_\nu, \\
H_1: f| \theta &\sim& T_\nu (\theta), \qquad \theta| \tau^2 \sim J(\tau^2, r), \quad \tau>0, \quad r \geq 1.
 \end{eqnarray}
\end{comment}
the marginal distribution of $M$ under $\mbox{H}_1$ can be expressed as:
{\footnotesize
\begin{align*}
   m_1(m)= 
   & \int m_0(m-\eta)\Bigg[\frac{1}{(1+\tau^2)^{r+\frac{1}{2}}}\ {_2}F_1\bigg(\frac{v+1}{2},\ r+\frac{1}{2},\ \frac{1}{2},\ \frac{\tau^2 (m-\eta)^2}{(t^2+\nu)(1+\tau^2)}\bigg)\\ 
   & + \frac{\tau (m-\eta)}{\sqrt{(m-\eta)^2+\nu}(1+\tau^2)^{r+1}}\ \frac{\Gamma\big(\frac{\nu}{2}+1\big)\ \Gamma(r+1)}{\Gamma\big(\frac{\nu+1}{2}\big)\ \Gamma\big(r+\frac{1}{2}\big)}\ {_2}F_1\ \bigg(\frac{\nu}{2}+1,\ r+1,\ \frac{3}{2},\ \frac{\tau^2 (m-\eta)^2}{(1+\tau^2)((m-\eta)^2+\nu)}\bigg)\Bigg]\ p(\eta) \ d\eta,
\end{align*}
}
and (ii) the marginal distribution of $M$ under the $\mbox{H}_0$ is given by:
\begin{eqnarray}
 m_0(m) = \int \frac{\Gamma\left(\frac{\nu + 1}{2}\right)}{\sqrt{\nu\pi}  \Gamma\left(\frac{\nu}{2}\right) \left(1 + \frac{(m-\eta)^2}{\nu}\right)^{-\frac{\nu+1}{2}}}\ p(\eta) \ d\eta \notag.
\end{eqnarray}
\end{proposition}
%\textcolor{red}{Please follow the Latex conventions in Lemmas \ref{eqn:bfbot_z} and \ref{eqn:bfbot_t} in sequel.}

\begin{proposition}[$\chi^2$-test]\label{eqn:bfbot_chi2}
Assume that the distribution of $f$ in \eqref{eqn:2.1} under the null and the alternative hypothesis are described as
\begin{align*}
\mbox{H}_0:  f\ \sim\ \chi^2_k ,\quad \text{against}\quad \mbox{H}_1: f\mid\theta\ \sim\ \chi^2_k(\theta), \quad \theta\mid \tau^2\ \sim\ G\Big(\frac{k}{2} + r,\ \frac{1}{2\tau^2}\Big), \quad \tau>0, \quad r \geq 1,.
\end{align*}
respectively. Then, (i) the marginal distribution of $M$ under $\mbox{H}_1$ can be expressed as:
\begin{align*} 
   m_1(m) = \int \frac{(m-\eta)^{\frac{k}{2}-1} \exp(-(m-\eta) / 2)}{2^{\frac{k}{2}} \Gamma(\frac{k}{2})\left(1+\tau^{2}\right)^{\frac{k}{2}+r}}\ {_1}F_1 \Bigg(\frac{k}{2}+r,\ \frac{k}{2},\ \frac{\tau^2 (m-\eta) }{2(1+\tau^2)}\Bigg))p(\eta) \ d\eta,
\end{align*}
and (ii) the marginal distribution of $M$ under the $\mbox{H}_0$ is given by:
\begin{eqnarray}
m_0(m) = \int \frac{1}{2^\frac{k}{2} \Gamma(\frac{k}{2})} (m-\eta)^{\frac{k}{2} - 1} \exp\bigg(-\frac{m-\eta}{2}\bigg)\ p(\eta) \ d\eta \nonumber.
\end{eqnarray}
\end{proposition}


\begin{proposition}[$F$-test]\label{eqn:bfbot_F}
Assume that the distribution of $f$ in \eqref{eqn:2.1} under the null and the alternative hypothesis are described as
\begin{align*}
\mbox{H}_0:  f\ \sim\ F_{k,\nu}(0) ,\quad \text{against}\quad \mbox{H}_1: f\mid\theta\ \sim\ F_{k,\nu}(\theta), \quad \theta\mid \tau^2\ \sim\ G\Big(\frac{k}{2}+r, \frac{1}{2\tau^2}\Big), \quad \tau>0, \quad r \geq 1,.
\end{align*}
respectively. Then, (i) the marginal distribution of $M$ under $\mbox{H}_1$ can be expressed as:
\begin{align*} 
   m_1(m) = \int \frac{m_0(m - \eta)}{(1+\tau^2)^{\frac{k}{2}+r}}\ {_2}F_{1}\Big(\frac{k+\nu}{2}, \frac{k}{2}+r,\ \frac{k}{2},\ \frac{k(m-\eta)\tau^2}{(\nu+k(m-\eta))(1+\tau^2)}\Big)\ p(\eta) \ d\eta,
\end{align*}
and (ii) the marginal distribution of $M$ under the $\mbox{H}_0$ is given by:
\begin{eqnarray}
m_0(m) = \int \frac{1}{\beta(\frac{k}{2},\frac{\nu}{2})}\Big(\frac{k}{\nu}\Big)^{\frac{k}{2}} (m-\eta)^{\frac{k}{2} - 1}\Big(1+\frac{k}{\nu}(m-\eta)\Big)^{-\frac{k+\nu}{2}} p(\eta) \ d\eta \nonumber.
\end{eqnarray}
\end{proposition}

\textcolor{red}{Need to include discussion on GSS, and choice of Bayes Factor cut offs. We may include results on Bayes Factor Consistency as remarks.}


\clearpage

